TExplain: Explaining Learned Visual Features via Pre-trained (Frozen) Language Models

Interpreting the learned features of vision models has posed a longstanding challenge in the field of machine learning. To address this issue, we propose a novel method that leverages the capabilities of language models to interpret the learned features of pre-trained image classifiers. Our method, called TExplain, tackles this task by training a neural network to establish a connection between the feature space of image classifiers and language models. Then, during inference, our approach generates a vast number of sentences to explain the features learned by the classifier for a given image. These sentences are then used to extract the most frequent words, providing a comprehensive understanding of the learned features and patterns within the classifier. Our method, for the first time, utilizes these frequent words corresponding to a visual representation to provide insights into the decision-making process of the independently trained classifier, enabling the detection of spurious correlations, biases, and a deeper comprehension of its behavior. To validate the effectiveness of our approach, we conduct experiments on diverse datasets, including ImageNet-9L and Waterbirds. The results demonstrate the potential of our method to enhance the interpretability and robustness of image classifiers.

==> ourcommands.tex <==


\newcommand{\noteam}[1]{%
    \todo[inline, size=\scriptsize, color=cyan!30]{#1}
}
\newcommand{\amnote}[1]{%
    \todo[line, tickmarkheight=0.1cm, size=\tiny, color=cyan!30]{#1}
} 
\newcommand{\am}[1]{\textcolor{orange}{#1}}
\newcommand{\methodname}{TExplain}


==> sections/broader_impact.tex <==
\section*{Broader Impact}

The findings and methodology presented in this paper have several implications and potential impacts on various stakeholders, including researchers, developers, and end-users of image classifiers and interpretable machine learning models.

\textbf{Advancements in Model Interpretability:} By introducing \methodname{} as a novel approach for interpreting pre-trained image classifiers, this work contributes to the ongoing efforts to enhance the interpretability of complex machine learning models. The ability to generate textual explanations that reveal learned features and patterns offers researchers and developers valuable insights into the decision-making process of image classifiers, facilitating model debugging, improvement, and further research in the field.

\textbf{Detection and Mitigation of Biases:} The capability of \methodname{} to detect and mitigate spurious correlations and biases within image classifiers has important implications for addressing fairness, transparency, and accountability in machine learning systems. The insights provided by \methodname{} can help identify unintended associations and biases that may arise during the training process, enabling developers to take corrective actions and improve the fairness and reliability of the classifiers.

\textbf{Improved Understanding of Model Behavior:} The comprehensive explanations generated by \methodname{} not only enhance the interpretability of image classifiers but also contribute to a deeper understanding of the underlying concepts and representations learned by these models. This understanding can lead to further insights and advancements in computer vision, enabling the development of more robust and accurate models for image classification tasks.

\textbf{Real-World Applications:} The practical applications of \methodname{} extend beyond research and development. The ability to interpret and understand the features learned by image classifiers has direct implications for real-world applications in areas such as healthcare, autonomous vehicles, surveillance systems, and content moderation. The insights gained from \methodname{} can help identify and address potential issues, ensuring that these systems operate in a reliable, unbiased, and safe manner.

\textbf{Ethical Considerations:} As with any advancements in machine learning interpretability, it is essential to consider and address ethical considerations and potential misuse of the proposed methodology. The responsible and ethical deployment of \methodname{} requires vigilance in avoiding unintended consequences, ensuring privacy protection, and preventing the amplification of existing biases or discrimination.

In summary, our proposed \methodname{} framework has the potential to impact the field of image classification and model interpretability by advancing our understanding of learned features, enabling bias detection, and enhancing transparency in decision-making. While the work offers significant contributions, it is crucial for researchers, developers, and policymakers to consider the broader impact and ethical considerations in the application and further development of \methodname{} to ensure its responsible and beneficial use in various domains.
